The mu-calculus' Alternation Hierarchy is Strict over Non-Trivial Fusion Logics

The modal mu-calculus is obtained by adding least and greatest fixed-point operators to modal logic. Its alternation hierarchy classifies the mu-formulas by their alternation depth: a measure of the codependence of their least and greatest fixed-point operators. The mu-calculus' alternation hierarchy is strict over the class of all Kripke frames: for all n, there is a mu-formula with alternation depth n+1 which is not equivalent to any formula with alternation depth n. This does not always happen if we restrict the semantics. For example, every mu-formula is equivalent to a formula without fixed-point operators over S5 frames. We show that the multimodal mu-calculus' alternation hierarchy is strict over non-trivial fusions of modal logics. We also comment on two examples of multimodal logics where the mu-calculus collapses to modal logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{Alexis Saurin (Editor): Fixed Points\\ 
in Computer Science 2024 (FICS 2024).\\
EPTCS 435, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.435.8}{10.4204/EPTCS.435.8}}
\pdfoutput=1

